A Lightweight Post-Quantum Authentication Framework for 5G Base Station Bootstrapping

The absence of authenticated bootstrapping between User Equipments (UEs) and Base Stations (BSs) in 5G leaves System Information Block (SIB) broadcasts unprotected, enabling fake BS attacks, man-in-the-middle interception, and spoofed emergency alerts. Prior efforts such as Public Key Infrastructure (PKI)-based certificate chains, token-based schemes, and identity-based signatures either impose overhead exceeding 5G's strict packet-size constraints or lack post-quantum (PQ) security. Direct NIST-PQC integration is also infeasible; current standards, such as ML-DSA requires 34 fragmented SIB1 packets and up to 5,282\,ms end-to-end delay, and FN-DSA still requires 13 fragments and up to 1,920\,ms. We propose EMULSION, a symmetric chained publicly verifiable authentication framework for 5G/6G BS broadcast authentication. EMULSION is the first framework to exploit native 5G architectural features: fixed SIB transmission windows, millisecond-level time synchronization, and eSIM/USIM credential management to achieve genuine PQ security at symmetric-key efficiency. It uses a timed stream loss-tolerant authentication with HMAC chain anchored by a compact PQ signature~(MAYO) applied once per epoch, fitting authentication within a single packet with no fragmentation and eliminating certificate transmission entirely. Unlike prior schemes, EMULSION extends to the full SIB family (SIB1-SIB21) at no additional per-broadcast cost, demonstrated over the air on SIB1. Evaluated on a real over-the-air 5G testbed, EMULSION achieves 33x lower end-to-end delay and 31x less communication overhead than ML-DSA, and 12x lower delay and 5.4x less overhead than FN-DSA. We formally prove the security of EMULSION and open-source its implementation for public testing and adaptation.

==> Chapters/Discussion.tex <==
\section{\blue{Discussion}} \label{sec:discussion}
% $\emulsion$ provides message-origin authentication for SIB broadcasts. The central point is that no adversary, whether in scope or out, can cause a UE to accept a forged SIB: forgery requires either a valid per-packet tag (and thus a chain key) or a valid anchor signature (and thus $\sk_\amf$), neither of which is available. Attacks outside our scope can therefore deny service, but cannot substitute authenticated content. 

% \textbf{Residual guarantees under out-of-scope attacks.} $\emulsion$ does not prevent physical-layer attacks. However, their effect is bounded to denial rather than deception. Under overshadowing, an adversary replaces a legitimate SIB with a forged one; lacking a valid tag or anchor signature, the forged packet fails verification and the UE aborts before RACH, so the attack yields a detected denial of service rather than a fraudulent attachment. Jamming and other physical-layer interference prevent delivery entirely, causing the UE to fail bootstrapping, as with any broadcast scheme, but never to attach to an unauthenticated cell. A relay that forwards genuine SIBs unmodified gains nothing, since the content remains authentic, while any modification invalidates the tag; a relay that instead delays packets is caught by the epoch-freshness check, which binds acceptance to receiver-side state rather than attacker-supplied timing. Denial-of-service at the MAC or RLC sublayer targets availability and is orthogonal to authentication. Across all these cases, $\emulsion$ reduces the adversary's capability from substituting system information to merely denying it.

% \noindent\textbf{$\emulsion$ in the overshadowing era.} Recent work on adaptive overshadowing~\cite{erni2022adaptover} shows that an over-the-air attacker can inject or replace arbitrary messages from kilometer range on live networks, achieving fake-base-station outcomes without deploying a base station, and argues that countermeasures focused on detecting rogue transmitters are no longer sufficient. $\emulsion$ is aligned with exactly this shift: its guarantee is not tied to identifying the transmitter but to authenticating the message. A forged SIB fails tag verification identically whether it originates from a rogue gNB or an overshadowing injector, so the arbitrary-injection capability that makes overshadowing powerful is reduced to detected denial. $\emulsion$ thus realizes the message-authenticating defense that transmitter-detection approaches cannot provide.

% \textbf{Compromise resilience and key management.} $\emulsion$ localizes the effect of compromise. A BS holds only the per-epoch chain material provisioned to it, not any long-term secret, so a compromised BS can forge SIBs only until the epoch expires, after which a fresh certified anchor supersedes it. This contrasts with PKI- and IBS-based schemes, where a leaked BS key remains usable until explicit revocation. Only the AMF root key requires lifecycle management: rotation is performed offline over the GSMA RSP channel already used for provisioning, with UEs holding the current and next key across a transition window, and revocation of the root is likewise an RSP update, avoiding per-BS revocation machinery. The remaining open case is cross-operator roaming: since trust is anchored in the home operator's pre-provisioned root, a visited network can be authenticated only if its root is provisioned in advance or cross-certified by the home operator; absent this, roaming falls back to unauthenticated SIBs as in current deployments. We treat authenticated roaming as future work.

\bfred{MIRZA, please add notes on these in the related section. I will remove this section as I merged my notes to the related sections.}

\noindent \bfblue{1. Add implemnetation results for other SIB Supports. Maybe SIB4,5,9. This would cover our claim for securing all the SIBs, so our implementation should not be limited to only SIB1.}

\noindent \bfblue{2. Time Synchronization Concern. Read the Rev's comments of Time Synchronization issues. We must add complementary notes to bypass this. Otherwise we get the same Review from NDSS.}

